Serenity: Library Based Python Code Analysis for Code Completion and Automated Machine Learning

Dynamically typed languages such as Python have become very popular. Among other strengths, Python's dynamic nature and its straightforward linking to native code have made it the de-facto language for many research areas such as Artificial Intelligence. This flexibility, however, makes static analysis very hard. While creating a sound, or a soundy, analysis for Python remains an open problem, we present in this work Serenity, a framework for static analysis of Python that turns out to be sufficient for some tasks. The Serenity framework exploits two basic mechanisms: (a) reliance on dynamic dispatch at the core of language translation, and (b) extreme abstraction of libraries, to generate an abstraction of the code. We demonstrate the efficiency and usefulness of Serenity's analysis in two applications: code completion and automated machine learning. In these two applications, we demonstrate that such analysis has a strong signal, and can be leveraged to establish state-of-the-art performance, comparable to neural models and dynamic analysis respectively.

==> sections/evaluation.tex <==
% \section{Validation of Analysis}
% The core research question we ask is whether Serenity produces any useful analysis outputs that can help applications that may benefit from such analysis; despite the challenges in modeling dynamic languages such as Python accurately.  We describe two specific uses of analysis below.  The automated machine learning use case examines if analysis artifacts can be used to automatically generate pipelines for machine learning.  
% % This work has an extensive series of experiments, and it has been submitted for publication, so we only sketch the main findings here\footnote{For purposes of anonymity, a full reference is not provided here, but will be in the final version, should the paper be accepted}.  
% We also examine a code completion use case, which we cover in more detail here because it is not described anywhere.

% \input{sections/code_generation}
% \input{sections/kgpip}
